OS-Oracle: A Comprehensive Framework for Cross-Platform GUI Critic Models

With VLM-powered computer-using agents (CUAs) becoming increasingly capable at graphical user interface (GUI) navigation and manipulation, reliable step-level decision-making has emerged as a key bottleneck for real-world deployment. In long-horizon workflows, errors accumulate quickly and irreversible actions can cause unintended consequences, motivating critic models that assess each action before execution. While critic models offer a promising solution, their effectiveness is hindered by the lack of diverse, high-quality GUI feedback data and public critic benchmarks for step-level evaluation in computer use. To bridge these gaps, we introduce OS-Oracle that makes three core contributions: (1) a scalable data pipeline for synthesizing cross-platform GUI critic data; (2) a two-stage training paradigm combining supervised fine-tuning (SFT) and consistency-preserving group relative policy optimization (CP-GRPO); (3) OS-Critic Bench, a holistic benchmark for evaluating critic model performance across Mobile, Web, and Desktop platforms. Leveraging this framework, we curate a high-quality dataset containing 310k critic samples. The resulting critic model, OS-Oracle-7B, achieves state-of-the-art performance among open-source VLMs on OS-Critic Bench, and surpasses proprietary models on the mobile domain. Furthermore, when serving as a pre-critic, OS-Oracle-7B improves the performance of native GUI agents such as UI-TARS-1.5-7B in OSWorld and AndroidWorld environments. The code is open-sourced at https://github.com/numbmelon/OS-Oracle.

==> tables/critic_agent_results.tex <==
\begin{table}[h]
  \centering
  \caption{Critic agent results.(chart is better)}
  \label{tab:critic_agent_results}
  \begin{tabular}{llcc}
    \toprule
    \textbf{Model} & \textbf{Critic Model} & \textbf{AW} & \textbf{OSWorld} \\
    \midrule
    \multirow{3}{*}{UI-TARS-1.5-7B} & - & 31.6  &  29.2 \\
    & GPT-4o &  30.2  &   28.5 \\
    & \name-7B & 33.2  &  31.0  \\

    \bottomrule
  \end{tabular}
\end{table}


==> tables/os_critic_bench_statistics.tex <==
\begin{table}[ht]
\centering
\small
\caption{
OS-Critic Bench Data Statistics. 
}
\scalebox{1}{
\begin{tabular}{l|cc}
    \toprule
    \textbf{Benchmarks} & \textbf{Platforms} &\textbf{\#Test Samples} \\
    \midrule
    GUI-Act-Web &Web &1,410  \\
    % \midrule
    % \multirow{2}{*}{Omniact} &Web &1,427 & &3+11 \\
    % & Desktop &594 & &3+11 \\
    % \midrule
    % AndroidControl-Low & Mobile &7,708 &\checkmark &3+5 \\
    % AndroidControl-High & Mobile &7,708 &\checkmark &3+5 \\
    % \midrule
    % GUI-Odyssey-Random &Mobile &29,414 & &3+6 \\
    % GUI-Odyssey-Task &Mobile &17,920 & &3+6 \\
    % GUI-Odyssey-Device &Mobile &18,969 & &3+6 \\
    % GUI-Odyssey-App &Mobile &17,455 & &3+6 \\
    % \bottomrule
\end{tabular}
}
\label{tab:os-critic-bench-statistics}
\end{table}

==> tables/sft_scaling.tex <==
\begin{table}[h]
  \centering
  \caption{SFT Data Scaling (Line chart later)}
  \label{tab:ablation_neg_results}
  \begin{tabular}{lcc}
    \toprule
    \textbf{Model} & \multicolumn{2}{c}{\textbf{Overall}} \\ 
    \cmidrule(lr){2-3}
    & \makecell[c]{Acc} & \makecell[c]{F1} \\
    \midrule
    Qwen2.5-VL & 58.27 & 66.23 \\
    10k & 57.59  & 67.29 \\
    50k & 60.03 & 69.37 \\
    100k & 60.43 & 68.12 \\
    all & 63.14 & 71.49 \\ 
    \bottomrule
  \end{tabular}
\end{table}

